Algebraic models of dependent type theory

The rules governing the essentially algebraic notion of a category with families have been observed (independently) by Steve Awodey and Marcelo Fiore to precisely match those of a representable natural transformation between presheaves. This provides us with a natural, functorial description of essentially algebraic objects which are used to model dependent type theory; following Steve Awodey, we call them 'natural models'. We can view natural models from several different viewpoints, of which we focus on three in this thesis. First, natural models are essentially algebraic, meaning that they can be described by specifying operations between sorts, subject to equational axioms; this allows us to assemble natural models into a category with certain beneficial properties. Second, since natural models are natural transformations between presheaves, they are morphisms in a locally cartesian closed category, meaning that they can be regarded as polynomials. Third, since natural models admit interpretations of dependent type theory, we can use them to provide a functorial semantics.

==> thesis/ch1-background/landscape.tex <==
\section{The landscape of categorical semantics}
\label{secLandscapeOfCategoricalSemantics}

In classical model theory, there is a single notion of `model' $\mathfrak{M}$ of a first-order theory $\mathbb{T}$, namely a set $M$ together with elements $c^{\mathfrak{M}} \in M$ for each constant symbol $c$ in $\mathbb{T}$, functions $f^{\mathfrak{M}} : M^n \to M$ for each function symbol $f$ in $\mathbb{T}$ of arity $n$, and subsets $R^{\mathfrak{M}} \subseteq M^n$ for each relation symbol $R$ in $\mathbb{T}$ of arity $n$, such that this data satisfies the formulae of $\mathbb{T}$.

For depenedent type theory, matters are complicated in several ways, not least that the propositions of the theory are themselves objects of the theory. As a result, many different notions of categorical model of dependent type theory have emerged, ranging from notions with strict structure that is very faithful to the syntax of dependent type theory, such as \textit{contextual categories} \cite{Cartmell1986GAT}, to notions with weaker structure that have a more homotopical flavour, such as \textit{clans} and \textit{tribes} \cite{Joyal2017ClansTribes}.

The notion explored in this thesis is that of a \textit{natural model} (\Cref{defNaturalModel}). Before exploring natural models, though, we will set the scene by describing some other approaches, which we will later connect with our own.

\subsection*{Grothendieck fibrations and comprehension categories}

As mentioned in \Cref{secTypesForTheWorkingMathematician}, the contexts and substitutions of a dependent type theory form the objects and morphisms, respectively, of a category $\mathbb{C}$. For each object $\Gamma$ of $\mathbb{C}$, 

\subsection*{Clans and tribes}


\subsection*{Categories with families}

==> thesis/ch2-categories-of-natural-models/other-notions-of-model.tex <==
\section{Situation amongst other notions of model}
\label{secOtherNotionsOfModel}

\todo{}

\subsection*{Categories with families}

\todo{}

\begin{theorem}[Natural models are categories with families are natural models]
\label{thmNMisoCWF}
The category $\mathbf{NM}$ of natural models is isomorphic to the category $\mathbf{CwF}$ of categories with families.
\end{theorem}

\begin{proof}
Natural models and categories with families are different presentations of models of the same essentially algebraic theory. \todo{Elaborate? Justify?}
\end{proof}

\todo{}

\begin{corollary}
The category $\mathbf{NM}$ is equivalent to the categories $\mathbf{CwA}$ of categories with attributes and $\mathbf{DiscCompCat}$ of discrete comprehension categories.
\end{corollary}

\begin{proof}
\todo{Cite relevant papers}
\end{proof}

\subsection*{Tribes}

\begin{definition}[Clans and tribes \thmcite{Joyal2017ClansTribes}]
\label{defClanTribe}
\index{clan}
\index{tribe}
\index{fibration!{---} in a clan/tribe}
\index{anodyne map!{---} in a clan/tribe}
A \textbf{clan} is a category $\mathcal{E}$ with a terminal object $1$ and a class $\mathcal{F} \subseteq \mathcal{E}$ of morphisms in $\mathcal{E}$ called \textbf{fibrations}, which satisfy the following closure properties:
\begin{enumerate}[(i)]
\item Every isomorphism in $\mathcal{E}$ is in $\mathcal{F}$;
\item $\mathcal{F}$ is closed under composition;
\item $\mathcal{F}$ is closed under pullbacks along arbitrary morphisms of $\mathcal{E}$; and
\item For each object $X$ of $\mathcal{E}$, the (unique) morphism $X \to 1$ to the terminal object is in $\mathcal{F}$.
\end{enumerate}
We write $\mathcal{A}$ for the class of morphisms in $\mathcal{E}$ with the left lifting property with respect to $\mathcal{F}$ and call the elements of $\mathcal{A}$ \textbf{anodyne maps}.

A clan $(\mathcal{E}, \mathcal{F})$ is a \textbf{tribe} if every morphism $f$ in $\mathcal{E}$ factors as $p \circ u$ for some fibration $p \in \mathcal{F}$ and anodyne map $u \in \mathcal{A}$, and if the class of anodyne maps is closed under pullbacks along arbitrary morphisms of $\mathcal{E}$.
\end{definition}

\todo{}

\begin{theorem}[Natural models are tribes]
Let $(\mathbb{C}, p)$ be a democratic natural model admitting a unit type and dependent sum types. The pair $(\mathbb{C}, \mathcal{F}_p)$ is a tribe, where $\mathcal{F}_p$ is the class of morphisms of $\mathbb{C}$ classified by $p$ (\Cref{defMorphismClassifiedByNM}). Moreover, the assignment $(\mathbb{C}, p) \mapsto (\mathbb{C}, \mathcal{F}_p)$ extends to a functor $\mathbf{NM}_{1,\Sigma,\mathrm{dem}} \to \mathbf{Trb}$.
\end{theorem}

\begin{proof}
First observe that $(\mathbb{C}, \mathcal{F}_p)$ is a clan. Indeed, $\mathcal{F}_p$ contains all isomorphisms and is closed under composition by \Cref{lemUnitsClassifyIsomorphisms,lemDependentSumsClassifyComposites}, since $(\mathbb{C}, p)$ admits a unit type and dependent sum types. Moreover $\mathcal{F}_p$ is closed under pullbacks along arbitrary morphisms of $\mathbb{C}$; this is an immediate consequence of the two pullbacks lemma. Finally, each morphism $\mathsf{t}_{\Gamma} : \Gamma \to \diamond$ is classified by $p$ since $(\mathbb{C}, p)$ is democratic---to see this, note that $(\Gamma, \mathsf{t}_{\Gamma}) \cong (\diamond \cext \bar{\Gamma}, \nmp{\bar{\Gamma}})$ in $\mathbb{C} \slice{\Gamma}$ and apply \Cref{lemClassificationOfMorphismsClassifiedByNM}.

\todo{Tribe?}

\todo{Extension to functor}
\end{proof}

\todo{}

\subsection*{Dominance}

\todo{}

\begin{definition}[Dominances \thmcite{Rosolini1986Continuity}]
\label{defDominance}
\index{dominance}
Let $\mathcal{E}$ be a category with a terminal object $1$. A \textbf{dominance} in $\mathcal{E}$ is a pair $(\Sigma, \top)$ consisting of an object $\Sigma$ and a subobject $\top : 1 \monoto \Sigma$, such that
\begin{enumerate}[(i)]
\item Pullbacks of $\top$ along arbitrary morphisms of $\mathcal{E}$ exist---such pullbacks are called \textbf{$\top$-subobjects};
\item Every $\top$-subobject arises uniquely as a pullback of $\top$, in the sense that for every $\top$-subobject $m : D \monoto A$, there is a unique morphism $\chi_m^{\top} : A \to \Sigma$, called the \textbf{characteristic morphism} of $m$, such that the following square is a pullback;
\begin{diagram}
D
\arrow[r]
\arrow[d, tail, "m"']
\pullback
&
1
\arrow[d, tail, "\top"]
\\
A
\arrow[r, "\chi_m^{\top}"']
&
\Sigma
\end{diagram}
\item The pullback functor $\top^* : \mathcal{E} \slice{\Sigma} \to \mathcal{E}$ has a right adjoint; and
\item The class of $\top$-subobjects is closed under composition.
\end{enumerate}
\end{definition}

\todo{}

\begin{theorem}[Natural models are dominances]
Let $(\mathbb{C}, p)$ be a natural model with underlying natural transformation $p : \Yon(\diamond) \to \nmty{U}$. If $(\mathbb{C}, p)$ admits dependent sum types, then $(\nmty{U}, p)$ is a dominance in $\widehat{\mathbb{C}}$.
\end{theorem}

\begin{proof}
Conditions (i) and (iii) of \Cref{defDominance} are satisfied immediately from the fact that $\widehat{\mathbb{C}}$ is a locally cartesian closed category. Condition (iv) is satisfied by the hypothesis that $(\mathbb{C}, p)$ admit dependent sum types \todo{State relevant result somewhere, refer to it.}
\end{proof}

==> thesis/files/cmu-seal.tex <==
%% Creator: Inkscape inkscape 0.91, www.inkscape.org
%% PDF/EPS/PS + LaTeX output extension by Johan Engelen, 2010
%% Accompanies image file 'cmu-seal.pdf' (pdf, eps, ps)
%%
%% To include the image in your LaTeX document, write
%%   \input{<filename>.pdf_tex}
%%  instead of
%%   \includegraphics{<filename>.pdf}
%% To scale the image, write
%%   \def\svgwidth{<desired width>}
%%   \input{<filename>.pdf_tex}
%%  instead of
%%   \includegraphics[width=<desired width>]{<filename>.pdf}
%%
%% Images with a different path to the parent latex file can
%% be accessed with the `import' package (which may need to be
%% installed) using
%%   \usepackage{import}
%% in the preamble, and then including the image with
%%   \import{<path to file>}{<filename>.pdf_tex}
%% Alternatively, one can specify
%%   \graphicspath{{<path to file>/}}
%% 
%% For more information, please see info/svg-inkscape on CTAN:
%%   http://tug.ctan.org/tex-archive/info/svg-inkscape
%%
\begingroup%
  \makeatletter%
  \providecommand\color[2][]{%
    \errmessage{(Inkscape) Color is used for the text in Inkscape, but the package 'color.sty' is not loaded}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\transparent[1]{%
    \errmessage{(Inkscape) Transparency is used (non-zero) for the text in Inkscape, but the package 'transparent.sty' is not loaded}%
    \renewcommand\transparent[1]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \ifx\svgwidth\undefined%
    \setlength{\unitlength}{240.0000071bp}%
    \ifx\svgscale\undefined%
      \relax%
    \else%
      \setlength{\unitlength}{\unitlength * \real{\svgscale}}%
    \fi%
  \else%
    \setlength{\unitlength}{\svgwidth}%
  \fi%
  \global\let\svgwidth\undefined%
  \global\let\svgscale\undefined%
  \makeatother%
  \begin{picture}(1,1)%
    \put(0,0){\includegraphics[width=\unitlength,page=1]{thesis/files/cmu-seal.pdf}}%
  \end{picture}%
\endgroup%

